SyncTweedies: A General Generative Framework Based on Synchronized Diffusions

We introduce a general framework for generating diverse visual content, including ambiguous images, panorama images, mesh textures, and Gaussian splat textures, by synchronizing multiple diffusion processes. We present exhaustive investigation into all possible scenarios for synchronizing multiple diffusion processes through a canonical space and analyze their characteristics across applications. In doing so, we reveal a previously unexplored case: averaging the outputs of Tweedie's formula while conducting denoising in multiple instance spaces. This case also provides the best quality with the widest applicability to downstream tasks. We name this case SyncTweedies. In our experiments generating visual content aforementioned, we demonstrate the superior quality of generation by SyncTweedies compared to other synchronization methods, optimization-based and iterative-update-based methods.

==> Rebuttal/diversity.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.7\linewidth]{Rebuttal/diversity.pdf}
    \caption{\textbf{Diversity comparison.} Optimization-based method Paint-it (Left) and diffusion-synchronization based method, SyncTweedies (Right). SyncTweedies generates more diverse images.}
    \label{result:mnist}
\end{figure}


==> Rebuttal/mnist.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.5\linewidth]{Rebuttal/mnist.pdf}
    \caption{\textbf{MNIST qualitative results.} Images generated from a diffusion model trained in the canonical space (left), and synchronized outputs of a diffusion model trained in the instance spaces (right).}
    \label{result:mnist}
\end{figure}


==> Rebuttal/space_complexity.tex <==
\begin{table}[t!]
\renewcommand{\arraystretch}{1.3}
\centering
\caption{\textbf{A space complexity comparison.} The best in each row is highlighted by \textbf{bold}.}
{
\scriptsize
\setlength{\tabcolsep}{0.2em}
\begin{tabularx}{\linewidth}{>{\centering}m{1.7cm} | >{\centering}m{2.5cm} | Y | Y | Y Y}
\toprule
Metric & Diffusion Synchronization & \makecell{Finetuning\\-Based} & 
\makecell{Optim.\\-Based} & \multicolumn{2}{c}{\makecell{Iter. View\\Updating}} \\
\cline{1-6}
\multirow{6}{*}{\makecell{VRAM Usage \\ (GiB) $\downarrow$ }} & \multicolumn{5}{c}{3D Mesh Texturing} \\
\cline{2-6}
& \makecell{\Ours{}\\Case 2} & \makecell{Paint3D} & {\makecell{Paint-it}} & {\makecell{TEXTure}} & {\makecell{Text2Tex}} \\
\cline{2-6}
& \textbf{6.49} & 9.15 & 28.36 & 10.66 & 10.92 \\
\cline{2-6}
& \multicolumn{5}{c}{3D Gaussian Splats Texturing} \\
\cline{2-6}
& \makecell{\Ours{}\\Case 2} & \makecell{-} & {\makecell{SDS}} & \multicolumn{2}{c}{\makecell{IN2N}} \\
\cline{2-6}
& 9.30 & - & \textbf{6.87} & \multicolumn{2}{c}{10.38} \\
\bottomrule
\end{tabularx}
}
\label{tbl:space_complexity}
\end{table}


==> Rebuttal/wide_image.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.90\linewidth]{Rebuttal/variation_view_prompts_v2.pdf}
    \caption{\textbf{View variations.} \texttt{SyncTweedies} can control view variations using varying prompts.}
    \label{result:mnist}
\end{figure}

